DialogueGCN: A Graph Convolutional Neural Network for Emotion Recognition in Conversation

Emotion recognition in conversation (ERC) has received much attention, lately, from researchers due to its potential widespread applications in diverse areas, such as health-care, education, and human resources. In this paper, we present Dialogue Graph Convolutional Network (DialogueGCN), a graph neural network based approach to ERC. We leverage self and inter-speaker dependency of the interlocutors to model conversational context for emotion recognition. Through the graph network, DialogueGCN addresses context propagation issues present in the current RNN-based methods. We empirically show that this method alleviates such issues, while outperforming the current state of the art on a number of benchmark emotion classification datasets.

==> data-results.tex <==
\begin{table*}[h!]
\centering
        \begin{tabular}{l|c|c|c|c|c|c}
            \toprule
            \multirow{2}{*}{Dataset}&\multicolumn{3}{c|}{$\#$ dialogues}&\multicolumn{3}{c}{$\#$ utterances}\\
            &train&val&test&train&val&test\\
            \hline \hline
            IEMOCAP&\multicolumn{2}{c|}{120}&31&\multicolumn{2}{c|}{5810}&1623\\
            AVEC&\multicolumn{2}{c|}{63}&32&\multicolumn{2}{c|}{4368}&1430\\
            MELD&1039&114&280& 9989& 1109& 2610\\
            % DailyDialog&11,118&1000&100&87,832&7912&7863\\
            EmoContext&30,159&2754&5508&90,477&8262&16,524\\
            \bottomrule
        \end{tabular}
    \caption{Trainig, validation and test data distribution in the datasets.}
        \label{table:data1}
\end{table*}


\begin{table*}[t]
	\centering
	\begin{tabular}{lccccc}
		\toprule

		Label & IEMOCAP & MELD & EmoContext\\
		\midrule
		Neutral & 1708 & 6436 & -\\
		Happiness/Joy & 648 & 2308 & 4669\\
		Surprise & - & 1636 & -\\
		Sadness & 1084 & 1002 & 5838\\
		Anger & 1103 & 1607 & 5954\\
		Disgust & - & 361 & -\\
		Fear & - & 358 & -\\
		Frustrated & 1849 & - & -\\
		Excited & 1041 & - & -\\
		Other & - & - & 21960\\
		\bottomrule
	\end{tabular}
	\caption{Label distribution statistics in the datasets.}
	\label{table:data2}
\end{table*}

% \begin{table*}[t]
% 	\centering
% 	\begin{tabular}{cccccc}
% 		\toprule

% 		Label & IEMOCAP & MELD & DailyDialog & EmoContext\\
% 		\midrule
% 		Neutral & 1708 & 6436 & 85572 & -\\
% 		Happiness/Joy & 648 & 2308 & 12885 & 4669\\
% 		Surprise & - & 1636 & 1823 & -\\
% 		Sadness & 1084 & 1002 & 1150 & 5838\\
% 		Anger & 1103 & 1607 & 1022 & 5954\\
% 		Disgust & - & 361 & 353 & -\\
% 		Fear & - & 358  & 74 & -\\
% 		Frustrated & 1849 & - & - & -\\
% 		Excited & 1041 & - & - & -\\
% 		Other & - & - & - & 21960\\
% 		\bottomrule
% 	\end{tabular}
% 	\caption{Label distribution statistics in the datasets.}
% 	\label{table:data2}
% \end{table*}


\begin{table*}[ht!]
  \centering
  \resizebox{\linewidth}{!}{
  % \tabcolsep=3pt
   \begin{tabular}{l||c@{~~}c|c@{~~}c|c@{~~}c|c@{~~}c|c@{~~}c|c@{~~}c|c@{~~}c}
    \hline
    \multirow{3}{*}{Methods} & \multicolumn{14}{c}{IEMOCAP}  \\
    \cline{2-15} & \multicolumn{2}{c|}{Happy} & \multicolumn{2}{c|}{Sad} &
                                        \multicolumn{2}{c|}{Neutral} & \multicolumn{2}{c|}{Angry} & \multicolumn{2}{c|}{Excited} & \multicolumn{2}{c|}{Frustrated} & \multicolumn{2}{c}{\textbf{Average(w)}}\\
    \cline{2-15} & Acc. & F1 & Acc. & F1 & Acc. & F1 & Acc. & F1 & Acc. & F1 & Acc. & F1 & Acc. & F1 \\
    \hline
    \hline
  CNN &27.77&29.86&57.14&53.83&34.33&40.14&61.17&52.44&46.15&50.09&62.99&55.75&48.92&48.18 \\
    Memnet &25.72&33.53&55.53&61.77&58.12&52.84&59.32&55.39&51.50&58.30&67.20&59.00&55.72&55.10\\
    bc-LSTM &29.17&34.43&57.14&60.87&54.17&51.81&57.06&56.73&51.17&57.95&67.19&58.92&55.21&54.95\\
    bc-LSTM+Att &30.56&35.63&56.73&62.90&57.55&53.00&59.41&59.24&52.84&58.85&65.88&59.41&56.32&56.19\\
    CMN &25.00&30.38&55.92&62.41&52.86&52.39&61.76&59.83&55.52&60.25&71.13&60.69&56.56&56.13 \\
    ICON &22.22&29.91&58.78&64.57&62.76&57.38&64.71&63.04&58.86&63.42&67.19&60.81&59.09&58.54\\
    \hline
    DialogueRNN &25.69&33.18&75.10&{\bf 78.80}&58.59&{\bf 59.21}&64.71&65.28&80.27&{\bf 71.86}&61.15&58.91&63.40&{\bf 62.75}\\
    DialogueGCN &40.62 &42.75 &89.14 &84.54 &61.92 &63.54 &67.53 &64.19 &65.46 &63.08 &64.18 &66.99 &65.25 &64.18\\
    \hline
   \end{tabular}
  }
  \caption{\label{results:IEMOCAP}}
\end{table*}

\begin{table}
% \scalebox{0.9}{
 \resizebox{\linewidth}{!}{
\centering
   \begin{tabular}{l||c@{~}c@{~}c@{~}c@{~}c}
    \hline
    \multirow{3}{*}{Methods} & \multicolumn{4}{c}{AVEC}\\
    \cline{2-5} &\multicolumn{1}{c}{Valence}& \multicolumn{1}{c}{Arousal}& \multicolumn{1}{c}{Expectancy} & \multicolumn{1}{c}{Power}\\
    \cline{2-5} & $MAE$ & $MAE$ & $MAE$ & $MAE$\\
    \hline
    \hline
  CNN &0.545&0.542&0.605&8.71 \\
    Memnet &0.202 &0.211&0.216&8.97\\
    bc-LSTM &0.194&0.212&0.201&8.90 \\
    bc-LSTM+Att &0.189&0.213&0.190&8.67 \\
    CMN &0.192&0.213&0.195&8.74 \\
    \hline
    DialogueRNN &0.168&0.165& 0.175&7.90\\
    DialogueGCN &{\bf 0.157}&{\bf 0.161}&{\bf 0.168}&{\bf 7.68}\\
    \hline
   \end{tabular}
   }
  \caption{\label{results:AVEC}}
  \end{table}
\begin{table}
\centering
   \begin{tabular}{l||c}
    \hline
    % Methods & F1  \\
    \multirow{2}{*}{Methods} & \multicolumn{1}{c}{MELD}\\
    \cline{2-} & F1 \\
    \hline
    \hline
    CNN & 55.02 \\
    bc-LSTM & 56.44\\
    bc-LSTM+Att &  56.70 \\
    \hline
    DialogueRNN & 57.03 \\
    DialogueGCN &  58.10\\
    \hline
   \end{tabular}
  \caption{\label{results:MELD}}
\end{table}


% \begin{table*}[ht!]
%   \centering
%   % \tabcolsep=3pt
%   \begin{tabular}{l||c}
%     \hline
%     Methods & F1  \\
%     \hline
%     \hline
%     CNN & 55.02 \\
%     bc-LSTM & 56.44\\
%     bc-LSTM+Att &  56.70 \\
%     DialogueRNN & 57.03 \\
%     DialogueGCN &  58.10\\
%     \hline
%   \end{tabular}
  
%   \caption{\label{results:MELD}}
% \end{table*}


\begin{table}[h]
\small
\begin{center}
% 	\centering
	\begin{tabular}{C{2cm}C{2.5cm}c}
		\toprule
		Sequential Encoder & Speaker-Level Encoder & F1  \\
		\midrule
		\cmark & \cmark &  64.18 \\
		\cmark & \xmark &  55.30 \\
		\xmark & \cmark &  56.71 \\
		\xmark & \xmark &  36.75 \\
		\bottomrule
	\end{tabular}
	\caption{Ablation results w.r.t the contextual encoder modules in IEMOCAP dataset.\label{table:abl1}}
\end{center}
\end{table}


\begin{table}[h]
\small
\begin{center}
% 	\centering
	\begin{tabular}{C{2.5cm}C{2.5cm}c}
		\toprule
		Speaker Dependency Edges & Temporal Dependency Edges & F1  \\
		\midrule
		\cmark & \cmark &  64.18 \\
		\cmark & \xmark &  62.52 \\
		\xmark & \cmark &  61.03 \\
		\xmark & \xmark &  60.11 \\
		\bottomrule
	\end{tabular}
	\caption{Ablation results w.r.t the edge relations in speaker-level encoder module in IEMOCAP dataset. \label{table:abl2}}
\end{center}
\end{table}
